Abstracting Event-Driven Systems with Lifestate Rules

We present lifestate rules--an approach for abstracting event-driven object protocols. Developing applications against event-driven software frameworks is notoriously difficult. One reason why is that to create functioning applications, developers must know about and understand the complex protocols that abstract the internal behavior of the framework. Such protocols intertwine the proper registering of callbacks to receive control from the framework with appropriate application programming interface (API) calls to delegate back to it. Lifestate rules unify lifecycle and typestate constraints in one common specification language. Our primary contribution is a model of event-driven systems from which lifestate rules can be derived. We then apply specification mining techniques to learn lifestate specifications for Android framework types. In the end, our implementation is able to find several rules that characterize actual behavior of the Android framework.

==> Makefile <==
######################################################################
# Makefile
#
# Makefile for LaTeX projects
######################################################################

BASE = main

PAPERS = $(BASE)
BIBS = $(wildcard *.orig.bib)
SRCS = $(wildcard *.tex) $(wildcard *.sty) $(BIBS:%.orig.bib=%.short.bib)

GS = gs
#GS = gswin32c

GS_OPTS = -q -dNOPAUSE -dBATCH -sDEVICE=bbox
DVIPS_OPTS = -Ppdf -Pcmz -Pamz -t letter -D 600 -G0
#DVIPS_OPTS = -t letter -z -P pdf
DVIPDFM_OPTS = -p letter
PS2PDF_OPTS = 

.PHONY: html dvi ps pdf all figeps figpdf

all: pdf
dvi: ${PAPERS:%=%.dvi}
${PAPERS:%=%.dvi}: ${SRCS} ${FIGURES:%=%.eps}
ps: ${PAPERS:%=%.ps}
pdf: ${PAPERS:%=%.pdf}
${PAPERS:%=%.pdf}: ${SRCS} ${FIGURES:%=%.pdf}
html: ${PAPERS:%=%/index.html}

clean:
	rm -rf ${PAPERS} ${PAPERS:%=%.dvi} ${PAPERS:%=%.ps} ${PAPERS:%=%.pdf} \
               auto builddate.tex *.aux *.toc *.lof *.lot *.log *.bbl *.blg \
               *.pst.* *.tmp *~ *.out *.thm *.detex *.tr.tex \
               *.short.bib

# Generate TR TeX
%.tr.tex: %.tex
	sed 's/\\TRfalse/\\TRtrue/' $< >$@

# Generate Posting Version TeX
%.post.tex: %.tex
	sed 's/\\Postingfalse/\\Postingtrue/' $< >$@

# Generate DVI
#   run once, then re-run until it's happy
#   input redirected from /dev/null is like hitting ^C at first error
%.dvi: %.tex
	${MAKE} figeps
	(echo -n "\def\builddate{"; date; echo "}") >builddate.tex
	if latex ${<} </dev/null; then \
		true; \
	else \
		stat=$$?; touch ${<:%.tex=%.dvi}; exit $$stat; \
	fi
	if grep -q "\\citation" ${<:%.tex=%.aux}; then \
		bibtex ${<:%.tex=%}; \
	fi
	while grep -q "Rerun to get" ${<:%.tex=%.log}; do \
		if latex ${<} </dev/null; then \
			true; \
		else \
			stat=$$?; touch ${<:%.tex=%.dvi}; exit $$stat; \
		fi; \
	done

# Generate PS
%.ps: %.dvi
	dvips ${DVIPS_OPTS} -o ${<:%.dvi=%.ps} $<

# Generate PDF
%.pdf: %.tex
	${MAKE} figpdf
	# Remove the .aux file because pdflatex wants it different
	rm -f ${<:%.tex=%.aux} ${<:%.tex=%.thm}
	(echo -n "\def\builddate{"; date; echo "}") >builddate.tex
	if pdflatex ${<} </dev/null; then \
		true; \
	else \
		stat=$$?; touch ${<:%.tex=%.pdf}; exit $$stat; \
	fi
	if grep -q "\\citation" ${<:%.tex=%.aux}; then \
		bibtex ${<:%.tex=%}; \
	fi
	while grep -q "Rerun to get" ${<:%.tex=%.log}; do \
		if pdflatex ${<} </dev/null; then \
			true; \
		else \
			stat=$$?; touch ${<:%.tex=%.pdf}; exit $$stat; \
		fi; \
	done

# Generate PDF (using dvipdfm)
#%.pdf: %.dvi
#	dvipdfm ${DVIPDFM_OPTS} $<

# Generate PDF (using ps2pdf)
#%.pdf: %.ps
#	ps2pdf ${PS2PDF_OPTS} $<

# Generate short bib
%.short.bib: %.orig.bib
	#sed -e 's/@string{SHORT/@string{/'
	sed -e 's/@string{SHORT/@string{/' \
            -e 's/[Ee]ditor/OPTeditor/' \
            -e 's/[Mm]onth/OPTmonth/' \
            -e 's/[Pp]ublisher/OPTpublisher/' \
            -e 's/[Aa]ddress/OPTaddress/' \
            -e 's/[Ii]sbn/OPTisbn/' \
            -e 's/[Ii]ssn/OPTissn/' \
            -e 's/^[ 	]*[Dd]oi/OPTdoi/' \
            -e 's/^[ 	]*[Uu]rl/OPTurl/' \
            -e 's/[Pp]ages/OPTpages/' \
            -e 's/[Cc]rossref/OPTcrossref/' \
            -e 's/[Ss]eries/OPTseries/' \
            $< > $@

%.txt: %.tex
	cat $< | detex | sed 's/---/--/g' > $@


==> bectex/Makefile <==
######################################################################
# Makefile
#
# Makefile for LaTeX projects
######################################################################

BASE = main

PAPERS = $(BASE)
BIBS = $(wildcard *.orig.bib)
SRCS = $(wildcard *.tex) $(wildcard *.sty) $(BIBS:%.orig.bib=%.short.bib)

GS = gs
#GS = gswin32c

GS_OPTS = -q -dNOPAUSE -dBATCH -sDEVICE=bbox
DVIPS_OPTS = -Ppdf -Pcmz -Pamz -t letter -D 600 -G0
#DVIPS_OPTS = -t letter -z -P pdf
DVIPDFM_OPTS = -p letter
PS2PDF_OPTS = 

.PHONY: html dvi ps pdf all figeps figpdf

all: pdf
dvi: ${PAPERS:%=%.dvi}
${PAPERS:%=%.dvi}: ${SRCS} ${FIGURES:%=%.eps}
ps: ${PAPERS:%=%.ps}
pdf: ${PAPERS:%=%.pdf}
${PAPERS:%=%.pdf}: ${SRCS} ${FIGURES:%=%.pdf}
html: ${PAPERS:%=%/index.html}

clean:
	rm -rf ${PAPERS} ${PAPERS:%=%.dvi} ${PAPERS:%=%.ps} ${PAPERS:%=%.pdf} \
               auto builddate.tex *.aux *.toc *.lof *.lot *.log *.bbl *.blg \
               *.pst.* *.tmp *~ *.out *.thm *.detex *.tr.tex \
               *.short.bib

# Generate TR TeX
%.tr.tex: %.tex
	sed 's/\\TRfalse/\\TRtrue/' $< >$@

# Generate Posting Version TeX
%.post.tex: %.tex
	sed 's/\\Postingfalse/\\Postingtrue/' $< >$@

# Generate DVI
#   run once, then re-run until it's happy
#   input redirected from /dev/null is like hitting ^C at first error
%.dvi: %.tex
	${MAKE} figeps
	(echo -n "\def\builddate{"; date; echo "}") >builddate.tex
	if latex ${<} </dev/null; then \
		true; \
	else \
		stat=$$?; touch ${<:%.tex=%.dvi}; exit $$stat; \
	fi
	if grep -q "\\citation" ${<:%.tex=%.aux}; then \
		bibtex ${<:%.tex=%}; \
	fi
	while grep -q "Rerun to get" ${<:%.tex=%.log}; do \
		if latex ${<} </dev/null; then \
			true; \
		else \
			stat=$$?; touch ${<:%.tex=%.dvi}; exit $$stat; \
		fi; \
	done

# Generate PS
%.ps: %.dvi
	dvips ${DVIPS_OPTS} -o ${<:%.dvi=%.ps} $<

# Generate PDF
%.pdf: %.tex
	${MAKE} figpdf
	# Remove the .aux file because pdflatex wants it different
	rm -f ${<:%.tex=%.aux} ${<:%.tex=%.thm}
	(echo -n "\def\builddate{"; date; echo "}") >builddate.tex
	if pdflatex ${<} </dev/null; then \
		true; \
	else \
		stat=$$?; touch ${<:%.tex=%.pdf}; exit $$stat; \
	fi
	if grep -q "\\citation" ${<:%.tex=%.aux}; then \
		bibtex ${<:%.tex=%}; \
	fi
	while grep -q "Rerun to get" ${<:%.tex=%.log}; do \
		if pdflatex ${<} </dev/null; then \
			true; \
		else \
			stat=$$?; touch ${<:%.tex=%.pdf}; exit $$stat; \
		fi; \
	done

# Generate PDF (using dvipdfm)
#%.pdf: %.dvi
#	dvipdfm ${DVIPDFM_OPTS} $<

# Generate PDF (using ps2pdf)
#%.pdf: %.ps
#	ps2pdf ${PS2PDF_OPTS} $<

# Generate short bib
%.short.bib: %.orig.bib
	#sed -e 's/@string{SHORT/@string{/'
	sed -e 's/@string{SHORT/@string{/' \
            -e 's/[Ee]ditor/OPTeditor/' \
            -e 's/[Mm]onth/OPTmonth/' \
            -e 's/[Pp]ublisher/OPTpublisher/' \
            -e 's/[Aa]ddress/OPTaddress/' \
            -e 's/[Ii]sbn/OPTisbn/' \
            -e 's/[Ii]ssn/OPTissn/' \
            -e 's/^[ 	]*[Dd]oi/OPTdoi/' \
            -e 's/^[ 	]*[Uu]rl/OPTurl/' \
            -e 's/[Pp]ages/OPTpages/' \
            -e 's/[Cc]rossref/OPTcrossref/' \
            -e 's/[Ss]eries/OPTseries/' \
            $< > $@

%.txt: %.tex
	cat $< | detex | sed 's/---/--/g' > $@


==> builddate.tex <==
-n \defuilddate{
Sat Dec 31 11:58:01 MST 2016
}


==> macros.tex <==
% -*-latex-*-
\makeatletter

\newcommand{\semname}{\ensuremath{\lambda_{\text{life}}}\xspace}
\newcommand{\toolname}{DroidLife\xspace}

%65 manual traces
%68 automatic traces
\newcommand{\numtraces}{133 }
\newcommand{\nummantraces}{65 }
\newcommand{\numautotraces}{68 }
\newcommand{\nobjects}{-1 }

\newcommand{\todoSM}[1]{\todo[inline,color=green!40]{{\bf Sergio: } #1}}


\newcommand{\obsbad}{\ensuremath{\hat{\mathbb{B}_o}}\xspace}
\newcommand{\obsall}{\ensuremath{\hat{\mathbb{T}_o}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Tikz Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{lastate}=[state,accepting,scale=0.3]
\tikzstyle{lainitial}=[initial,initial text={}, initial where=above]
\tikzstyle{lalabel}=[scale=1]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Listing Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Syntax
\lstdefinelanguage{Enable}{
  morekeywords={let,in,if,then,else,new,bind,invoke,enable,disable,allow,disallow,fun,true,false,me,app,fwk,event,callback,callin,force},
  literate={skip}{{$\bullet$}}1
}

\newcommand{\cbstyle}{\colordullx{0}\slshape}
\newcommand{\cistyle}{\colordullx{4}}
\newcommand{\fwktystyle}{\colordullx{1}\itshape\relsize{-1}}
\newcommand{\evtstyle}{\normalfont\ttfamily\scshape}
\lstdefinelanguage{exthighlighting}[]{highlighting}{%
  moredelim=**[is][\cbstyle]{|cb:}{|},
  moredelim=**[is][\cistyle]{|ci:}{|},
  moredelim=**[is][\fwktystyle]{|fwkty:}{|},
  moredelim=*[is][\evtstyle]{|evt:}{|}
}

\lstset{
  emphstyle=\cbstyle,
  emph={onCreate,onResume,onPause,onDestroy,onClick,onPrepared,onError,doInBackground},
  emphstyle={[2]\cistyle},
  emph={[2]setOnClickListener,setOnPreparedListener,reset,start,setEnabled,enable,disable,setDataSource,prepareAsync,execute,cancel,<init>,getResources,getWidth},
  emphstyle={[3]\fwktystyle},
  emph={[3]Activity,Button,AsyncTask,OnClickListener,View, Fragment}
}

\newcommand{\codej}[1]{\codex{language=Java,alsolanguage=exthighlighting}{#1}}
\newcommand{\coden}[1]{\codex{language=Enable,alsolanguage=exthighlighting}{#1}}
\newcommand{\enmkkw}[2]{\sbox#1{\coden{#2}}}

\newcommand{\codejmk}[3][\relax]{\sbox#2{#1\codej{#3}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Concrete Model
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\subst}[2]{\ensuremath{[#1/#2]}}

% Maps
\newcommand{\map}[1]{\ensuremath{[#1]}}
\newcommand{\maplet}[2]{\ensuremath{#1 \mathbin{\mapsto} #2}}
%\newcommand{\empmap}{\ensuremath{\map{\,}}}
\newcommand{\empmap}{\ensuremath{\cdot}}
\newcommand{\extmap}[2]{\ensuremath{[\maplet{#1}{#2}]}}
\newcommand{\MapST}[2]{\ensuremath{\left[\,#1 \SuchThat{#1}{#2} #2\,\right]}}

%%% Meta Variables
\newcommand{\term}{\ensuremath{t}}
\newcommand{\expr}{\ensuremath{e}}
\newcommand{\ExprSet}{\SetName{Expr}}
\newcommand{\var}{\ensuremath{x}}
\newcommand{\VarSet}{\SetName{Var}}
\newcommand{\fld}{\ensuremath{f}}
\newcommand{\FldSet}{\SetName{Field}}
\newcommand{\fun}{\ensuremath{\lambda}}
\newcommand{\cont}{\ensuremath{k}}
\newcommand{\ContSet}{\SetName{Cont}}
\newcommand{\val}{\ensuremath{v}}
\newcommand{\ValSet}{\SetName{Val}}
\newcommand{\addr}{\ensuremath{a}}
\newcommand{\AddrSet}{\SetName{Addr}}
\newcommand{\thunk}{\ensuremath{\kappa}}
\newcommand{\ThunkSet}{\SetName{Thunk}}
\newcommand{\handle}{\ensuremath{h}}
\newcommand{\HandleSet}{\SetName{Handle}}
\newcommand{\msg}{\ensuremath{m}}
\newcommand{\MsgSet}{\SetName{Msg}}
\newcommand{\pkg}{\ensuremath{g}}
\newcommand{\trans}{\ensuremath{\tau}}
\newcommand{\transset}{\ensuremath{T}}
\newcommand{\TransSet}{\SetName{Trans}}
\newcommand{\absTransSet}{\absofset{\TransSet}}
\newcommand{\observe}{\ensuremath{o}}
\newcommand{\ObserveSet}{\SetName{Observable}}
\newcommand{\obsty}{\MVar{oknd}}
\newcommand{\directive}{\ensuremath{r}}
\newcommand{\directiveset}{\ensuremath{R}}
\newcommand{\absrule}{\absof{\directive}}
\newcommand{\absrules}{\absof{\directiveset}}
\newcommand{\DirectiveSet}{\SetName{Cmd}}
\newcommand{\statepath}{\ensuremath{\pi}}
\newcommand{\statepathset}{\ensuremath{\Pi}}
\newcommand{\PathSet}{\SetName{Path}}
\newcommand{\trace}{\ensuremath{\varpi}}
\newcommand{\abstrace}{\ensuremath{\absof{\trace}}}
\newcommand{\traceset}{\ensuremath{\varPi}}
\newcommand{\abstraceset}{\ensuremath{\absof{\traceset}}}
\newcommand{\TraceSet}{\SetName{Trace}}
\newcommand{\absTransSeqSet}{\ensuremath{\seqof{\absofset{\TransSet}}}}
\newcommand{\obstrace}{\ensuremath{\theta}}
\newcommand{\obstraceset}{\ensuremath{\Theta}}
\newcommand{\ObsTraceSet}{\SetName{Observ}}
\newcommand{\SpecSet}{\SetName{LifeSpec}}
\newcommand{\weight}{\ensuremath{w}}
\newcommand{\tytag}{\ensuremath{T}}
\newcommand{\TytagSet}{\SetName{Tag}}

\newcommand{\Specmine}{\operatorname{spec\_mine}}

\newcommand{\env}{\ensuremath{\eta}}
\newcommand{\EnvSet}{\SetName{Env}}
\newcommand{\store}{\ensuremath{\rho}}
\newcommand{\StoreSet}{\SetName{Store}}
\newcommand{\eventmap}{\ensuremath{\mu}}
\newcommand{\EventmapSet}{\SetName{Enabled}}
\newcommand{\callinmap}{\ensuremath{\nu}}
\newcommand{\CallinmapSet}{\SetName{Allowed}}

\newcommand{\fmtevt}[1]{\ensuremath{\text{\evtstyle #1}}}
\newcommand{\evtcb}[2]{\enFrame{\fmtevt{#1}}{#2}}

\newcommand{\state}{\ensuremath{\sigma}}
\newcommand{\StateSet}{\SetName{State}}

\newsavebox{\@enkwLet}\enmkkw{\@enkwLet}{let}
\newcommand{\enkwLet}{\usebox{\@enkwLet}}
\newsavebox{\@enkwIn}\enmkkw{\@enkwIn}{in}
\newcommand{\enkwIn}{\usebox{\@enkwIn}}
\newsavebox{\@enkwIf}\enmkkw{\@enkwIf}{if}
\newcommand{\enkwIf}{\usebox{\@enkwIf}}
\newsavebox{\@enkwThen}\enmkkw{\@enkwThen}{then}
\newcommand{\enkwThen}{\usebox{\@enkwThen}}
\newsavebox{\@enkwElse}\enmkkw{\@enkwElse}{else}
\newcommand{\enkwElse}{\usebox{\@enkwElse}}
\newsavebox{\@enkwNew}\enmkkw{\@enkwNew}{new}
\newcommand{\enkwNew}{\usebox{\@enkwNew}}
\newsavebox{\@enkwBind}\enmkkw{\@enkwBind}{bind}
\newcommand{\enkwBind}{\usebox{\@enkwBind}}
\newsavebox{\@enkwInvoke}\enmkkw{\@enkwInvoke}{invoke}
\newcommand{\enkwInvoke}{\usebox{\@enkwInvoke}}
\newsavebox{\@enkwEnable}\enmkkw{\@enkwEnable}{enable}
\newcommand{\enkwEnable}{\usebox{\@enkwEnable}}
\newsavebox{\@enkwDisable}\enmkkw{\@enkwDisable}{disable}
\newcommand{\enkwDisable}{\usebox{\@enkwDisable}}
\newsavebox{\@enkwAllow}\enmkkw{\@enkwAllow}{allow}
\newcommand{\enkwAllow}{\usebox{\@enkwAllow}}
\newsavebox{\@enkwDisallow}\enmkkw{\@enkwDisallow}{disallow}
\newcommand{\enkwDisallow}{\usebox{\@enkwDisallow}}
\newsavebox{\@enkwFun}\enmkkw{\@enkwFun}{fun}
\newcommand{\enkwFun}{\usebox{\@enkwFun}}
\newsavebox{\@enkwForce}\enmkkw{\@enkwForce}{force}
\newcommand{\enkwForce}{\usebox{\@enkwForce}}
\newsavebox{\@enkwTrue}\enmkkw{\@enkwTrue}{true}
\newcommand{\enkwTrue}{\usebox{\@enkwTrue}}
\newsavebox{\@enkwFalse}\enmkkw{\@enkwFalse}{false}
\newcommand{\enkwFalse}{\usebox{\@enkwFalse}}
\newsavebox{\@enkwMe}\enmkkw{\@enkwMe}{me}
\newcommand{\enkwMe}{\usebox{\@enkwMe}}
\newsavebox{\@enkwApp}\enmkkw{\@enkwApp}{app}
\newcommand{\enkwApp}{\usebox{\@enkwApp}}
\newsavebox{\@enkwFwk}\enmkkw{\@enkwFwk}{fwk}
\newcommand{\enkwFwk}{\usebox{\@enkwFwk}}
\newsavebox{\@enkwEvent}\enmkkw{\@enkwEvent}{event}
\newcommand{\enkwEvent}{\usebox{\@enkwEvent}}
\newsavebox{\@enkwCallback}\enmkkw{\@enkwCallback}{callback}
\newcommand{\enkwCallback}{\usebox{\@enkwCallback}}
\newsavebox{\@enkwCallin}\enmkkw{\@enkwCallin}{callin}
\newcommand{\enkwCallin}{\usebox{\@enkwCallin}}

\newcommand{\fmtstate}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\enkwDisallowed}{\fmtstate{disallowed}}
\newcommand{\enkwInitial}{\fmtstate{initial}}

\newcommand{\enLet}[3]{\ensuremath{\enkwLet\;#1\;\pcode{=}\;#2\;\enkwIn\;#3}}
\newcommand{\enGetf}[2]{\ensuremath{#1\pcode{.}#2}}
\newcommand{\enPutf}[3]{\ensuremath{#1\pcode{.}#2\;\pcode{=}\;#3}}
\newcommand{\enNew}{\enkwNew}
\newcommand{\enSkipK}{\ensuremath{\bullet}}
\newcommand{\enSkip}{\ensuremath{()}}
\newcommand{\enSeq}[2]{\ensuremath{#1\pcode{;}\,#2}}
\newcommand{\enIf}[3]{\ensuremath{\enkwIf\;#1\;\enkwThen\;#2\;\enkwElse\;#3}}
\newcommand{\enBind}[2]{\ensuremath{\enkwBind\;#1\;#2}}
\newcommand{\enInvoke}[2]{\ensuremath{\enkwInvoke\;#1\;#2}}
\newcommand{\enEnable}[1]{\ensuremath{\enkwEnable\;#1}}
\newcommand{\enDisable}[1]{\ensuremath{\enkwDisable\;#1}}
\newcommand{\enAllow}[1]{\ensuremath{\enkwAllow\;#1}}
\newcommand{\enDisallow}[1]{\ensuremath{\enkwDisallow\;#1}}
\newcommand{\enFun}[3][\pkg]{\ensuremath{\enkwFun_{#1}\;#2\;\enkwIn\;#3}}
\newcommand{\enForce}[1]{\ensuremath{\enkwForce\;#1}}
\newcommand{\enTrue}{\enkwTrue}
\newcommand{\enFalse}{\enkwFalse}
\newcommand{\enMe}{\enkwMe}
\newcommand{\enApp}{\enkwApp}
\newcommand{\enAppSub}{\ensuremath{\mathbf{app}}}
\newcommand{\enFwk}{\enkwFwk}
\newcommand{\enFwkSub}{\ensuremath{\mathbf{fwk}}}
%\newcommand{\enEvent}[1]{\ensuremath{\enkwEvent\;#1}}
%\newcommand{\enCallback}[1]{\ensuremath{\enkwCallback\;#1}}
%\newcommand{\enCallin}[1]{\ensuremath{\enkwCallin\;#1}}
\newcommand{\enEvent}{\enkwEvent}
\newcommand{\enCallin}{\enkwCallin}
\newcommand{\enInitial}{\enkwInitial}
\newcommand{\enDisallowed}{\enkwDisallowed}
\newcommand{\enCallback}{\enkwCallback}

%\newcommand{\enClosure}[2]{\ensuremath{#1[#2]}}
\newcommand{\enClosure}[2]{\ensuremath{#1}}
\newcommand{\enMsg}[2]{\ensuremath{(#1,#2)}}
\newcommand{\extMsg}[2]{\ensuremath{[\enMsg{#1}{#2}]}}
%\newcommand{\ext}[1]{\ensuremath{[#1]}}
\newcommand{\ext}[1]{\ensuremath{, #1}}
%\newcommand{\enMsg}[2]{\ensuremath{#1 #2}}
\newcommand{\enThunk}[2]{\ensuremath{#1[#2]}}
\newcommand{\frameop}{\mathord{\gg}}
\newcommand{\enFrame}[2]{\ensuremath{#1\frameop#2}}

\newcommand{\enLetK}[4]{\ensuremath{\enkwLet\;#1\;\pcode{=}\;#2\;\enkwIn\;#3}}

\newcommand{\@enState}{}
%\long\def\@enState[#1][#2][#3][#4][#5][#6]{\ensuremath{\tuple{#1, #2, #3, #4, #5, #6}}}
\long\def\@enState[#1][#2][#3][#4][#5][#6]{\ensuremath{\tuple{#1, #3, #4, #5, #6}}}
\newcommand{\enState}{\optparams{\@enState}{[\expr][\env][\store][\eventmap][\callinmap][\cont]}}

\newcommand{\@enSigState}{}
\long\def\@enSigState[#1][#2][#3]{\ensuremath{\tuple{#1, #2, #3}}}
\newcommand{\enSigState}{\optparams{\@enSigState}{[\absof{\trace}][\absof{\eventmap}][\absof{\callinmap}]}}


\newcommand{\Package}{\operatorname{pkg}}
\newcommand{\Msg}{\operatorname{msg}}

\newcommand{\fmttrans}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\enkwInit}{\fmttrans{init}}
\newcommand{\enkwEvt}{\fmttrans{evt}}
\newcommand{\enkwCb}{\fmttrans{cb}}
\newcommand{\enkwCi}{\fmttrans{ci}}
\newcommand{\enkwDis}{\fmttrans{dis}}
\newcommand{\enkwRet}{\fmttrans{ret}}
\newcommand{\enkwFin}{\fmttrans{fin}}
\newcommand{\enObs}[2]{\ensuremath{#1\;#2}}
\newcommand{\enInit}{\fmttrans{init}}
\newcommand{\enEvt}[1]{\ensuremath{\enkwEvt\;#1}}
\newcommand{\enCb}[1]{\ensuremath{\enkwCb\;#1}}
\newcommand{\enCi}[1]{\ensuremath{\enkwCi\;#1}}
\newcommand{\enDis}[1]{\ensuremath{\enkwDis\;#1}}
\newcommand{\enRet}[1]{\ensuremath{\enkwRet\;#1}}
\newcommand{\enFin}[1]{\ensuremath{\enkwFin\;#1}}
\newcommand{\silentTrans}{\ensuremath{\varepsilon}}

\newcommand{\@displaydiamond}{\scalebox{1.17}[0.87]{$\displaystyle\Diamond$}}
\newcommand{\@textdiamond}{\scalebox{1.17}[0.87]{$\textstyle\Diamond$}}
\newcommand{\@scriptdiamond}{\scalebox{1.15}[0.87]{$\scriptstyle\Diamond$}}
\newcommand{\@scriptscriptdiamond}{\scalebox{1.11}[0.87]{$\scriptscriptstyle\Diamond$}}

\newcommand{\diamondplus}{\mathbin{\mathchoice%
{\ooalign{\@displaydiamond\cr\hidewidth$\displaystyle+$}}%
{\ooalign{\@textdiamond\cr\hidewidth$\textstyle+$}}%
{\ooalign{\@scriptdiamond\cr\hidewidth$\scriptstyle+$}}%
{\ooalign{\@scriptscriptdiamond\cr\hidewidth$\scriptscriptstyle+$}}%
}}
\newcommand{\diamondminus}{\mathbin{\mathchoice%
{\ooalign{\@displaydiamond\cr\hidewidth$\displaystyle-$}}%
{\ooalign{\@textdiamond\cr\hidewidth$\textstyle-$}}%
{\ooalign{\@scriptdiamond\cr\hidewidth$\scriptstyle-$}}%
{\ooalign{\@scriptscriptdiamond\cr\hidewidth$\scriptscriptstyle-$}}%
}}

%\newcommand{\specArrow}{\mathord{\shortrightarrow}}
\newcommand{\specArrow}{\mathord{\rightarrow}}
\newcommand{\nspecArrow}{\mathord{\nrightarrow}}
%\newcommand{\specEnableOp}{\mathop{\diamondplus}}
\newcommand{\specEnableOp}{\mathop{\text{\relsize{-1}\enkwEvt}}}
%\newcommand{\specDisableOp}{\mathop{\diamondminus}}
\newcommand{\specDisableOp}{\mathop{\text{\relsize{-1}\enkwEvt}}}
%\newcommand{\specAllowOp}{\mathop{\boxplus}}
\newcommand{\specAllowOp}{\mathop{\text{\relsize{-1}\enkwCi}}}
%\newcommand{\specDisallowOp}{\mathop{\boxminus}}
\newcommand{\specDisallowOp}{\mathop{\text{\relsize{-1}\enkwCi}}}

\newcommand{\specEnable}[3][]{\ensuremath{#2 \specArrow_{#1} \specEnableOp #3}}
\newcommand{\specDisable}[3][]{\ensuremath{#2 \nspecArrow_{#1} \specDisableOp #3}}
\newcommand{\specAllow}[3][]{\ensuremath{#2 \specArrow_{#1} \specAllowOp #3}}
\newcommand{\specDisallow}[3][]{\ensuremath{#2 \nspecArrow_{#1} \specDisallowOp #3}}

\newcommand{\allSpecs}[4]{\ensuremath{{#3}_{\joinrel{#1}{#2}}(#4)}}
\newcommand{\allEnables}[1]{\allSpecs{\specArrow}{\specEnableOp}{}{#1}}
\newcommand{\allDisables}[1]{\allSpecs{\nspecArrow}{\specDisableOp}{}{#1}}
\newcommand{\allAllows}[1]{\allSpecs{\specArrow}{\specAllowOp}{}{#1}}
\newcommand{\allDisallows}[1]{\allSpecs{\nspecArrow}{\specDisallowOp}{}{#1}}
\newcommand{\allRules}[1]{\allSpecs{\dashrightarrow}{}{}{#1}}

\newcommand{\specPermit}[3][]{\ensuremath{#2 \specArrow_{#1} #3}}
\newcommand{\specForbid}[3][]{\ensuremath{#2 \nspecArrow_{#1} #3}}


\newcommand{\Trace}{\operatorname{tr}}
\newcommand{\Observe}{\operatorname{obs}}
\newcommand{\Args}{\operatorname{args}}
\newcommand{\EvtArgs}{\operatorname{xargs}}
\newcommand{\Partition}{\operatorname{parti}}
\newcommand{\Callbacks}{\operatorname{evtcbs}}
\newcommand{\Elimci}{\operatorname{elimci}}

\newcommand{\slicectx}{\ensuremath{\Delta}}
\newcommand{\traceslice}[3][\slicectx]{\ensuremath{#2 \upharpoonright_{#3}^{#1}}}

%%% Judgments
\newcommand{\jstep}[3][]{\ensuremath{#2 \longrightarrow_{#1} #3}}
%\newcommand{\jstepins}[3][\trans]{\ensuremath{#2 \stackrel{\text{\normalsize$\longrightarrow$}}{\text{\scriptsize$#1$}} #3}}
\newcommand{\insstep}[1]{\mathrel{\ooalign{\raise0.25ex\hbox{$\longrightarrow$}\cr\hfil\raise-0.35ex\hbox{\relsize{-1}$#1$}\hfil}}}
\newcommand{\jstepins}[3][\trans]{\ensuremath{#2 \insstep{#1} #3}}

\newcommand{\jcaption}[1]{\hfill\fbox{\normalsize$#1$}}

%%% Abstraction
\newcommand{\absmsg}{\absof{\msg}}
\newcommand{\absforce}{\absof{\imath}}
\newcommand{\initforce}{\mathsf{init}}

\newcommand{\abselem}{\ensuremath{\AIabselementfn}}
\newcommand{\absconc}{\ensuremath{\absof{\AIconcfn}}}
\newcommand{\conc}{\ensuremath{\AIconcfn}}


%%% Spec learning
%\newcommand{\hmm}{\emph{HMM}}
\newcommand{\hmm}{HMM\xspace}
\newcommand{\pfsa}{\ensuremath{\text{\rm PFSA}}\xspace}
\newcommand{\mc}{MC\xspace}
\newcommand{\sharpsat}{\ensuremath{\sharp\text{SAT}}\xspace}
\newcommand{\Alphabet}{\ensuremath{\Sigma}}
\newcommand{\AlphabetCi}{\ensuremath{\Sigma_{\enkwCi}}}
\newcommand{\AlphabetCb}{\ensuremath{\Sigma_{\enkwEvt}}}
\newcommand{\RuleSet}{\ensuremath{RuleSet}}

%%% SharpSat
\newcommand{\abspath}{\ensuremath{\absof{\statepath}}}
\newcommand{\nondet}{\ensuremath{\text{\rm n}}}
\newcommand{\Card}[1]{\ensuremath{|{#1}|}}
\newcommand{\TraceFreq}[3]{\ensuremath{\SetName{Freq}({#1},{#2},{#3})}}
\newcommand{\threshold}{\ensuremath{\delta}}
\newcommand{\AbsPaths}[1]{\ensuremath{\SetName{Paths}({#1})}}
\newcommand{\AbsPathsRule}[2]{\ensuremath{\SetName{RulePaths}({#1},{#2})}}

%%% SharpSAT Encoding
\newcommand{\EncAbsPaths}[1]{\ensuremath{\SetName{EncPaths}({#1})}}
\newcommand{\EncAbsPathsRule}[2]{\ensuremath{\SetName{EncRulePaths}({#1},{#2})}}

%%% state var for a
\newcommand{\allvars}{\ensuremath{V}}
\newcommand{\statevarset}[1]{\ensuremath{X^{{#1}}}}
\newcommand{\statevar}[2]{\ensuremath{x_{{#1}}^{{#2}}}}
\newcommand{\permitset}[1]{\ensuremath{P^{{#1}}}}
\newcommand{\permitvar}[2]{\ensuremath{p_{{#1}}^{{#2}}}}
\newcommand{\prohibitset}[1]{\ensuremath{D^{{#1}}}}
\newcommand{\prohibitvar}[2]{\ensuremath{d_{{#1}}^{{#2}}}}

\newcommand{\actionenc}[2]{\ensuremath{Act({#1},{#2})}}
\newcommand{\encdis}[1]{\ensuremath{Dis({#1})}}
\newcommand{\encperm}[1]{\ensuremath{Perm({#1})}}

\makeatother

